SSA-COMET: Do LLMs Outperform Learned Metrics in Evaluating MT for Under-Resourced African Languages?

Evaluating machine translation (MT) quality for under-resourced African languages remains a significant challenge, as existing metrics often suffer from limited language coverage and poor performance in low-resource settings. While recent efforts, such as AfriCOMET, have addressed some of the issues, they are still constrained by small evaluation sets, a lack of publicly available training data tailored to African languages, and inconsistent performance in extremely low-resource scenarios. In this work, we introduce SSA-MTE, a large-scale human-annotated MT evaluation (MTE) dataset covering 14 African language pairs from the News domain, with over 73,000 sentence-level annotations from a diverse set of MT systems. Based on this data, we develop SSA-COMET and SSA-COMET-QE, improved reference-based and reference-free evaluation metrics. We also benchmark prompting-based approaches using state-of-the-art LLMs like GPT-4o, Claude-3.7 and Gemini 2.5 Pro. Our experimental results show that SSA-COMET models significantly outperform AfriCOMET and are competitive with the strongest LLM Gemini 2.5 Pro evaluated in our study, particularly on low-resource languages such as Twi, Luo, and Yoruba. All resources are released under open licenses to support future research.

==> tables/main_results_QE_Pearson.tex <==
% \begin{table*}[htbp]
% \centering
% \large
% \resizebox{1.05\textwidth}{!}{%
% \begin{tabular}{l|ccc|ccccc|cc}
% \toprule
% \makecell[l]{Language\\Pair}  & \makecell[c]{Gemini-2.0\\flash} & \makecell[c]{GPT-4o\\5shots} & \makecell[c]{Claude-3.7\\5shots} & CometKiwi & AfriCOMETv1.1-QE & AfriCOMETv1.0-MTL & AfriCOMETv1.1-MTL & Metric-X24 & SSA-COMET-QE & SSA-COMET-MTL \\
% \midrule
% eng-kik   & 0.5856 & 0.5431 & 0.6088 & 0.2986 & 0.5816 & 0.3774 & 0.6481 & 0.4520 & 0.6555 & \textbf{0.7340} \\
% eng-luo   & 0.6126 & 0.5761 & 0.6457 & 0.1755 & 0.5599 & 0.2592 & 0.6385 & 0.3321 & 0.6497 & 0.7324 \\
% fra-wol   & 0.6247 & 0.5831 & 0.6231 & 0.2358 & 0.3989 & 0.2644 & 0.3583 & 0.2583 & 0.5765 & 0.6358 \\
% fra-ewe   & 0.5017 & 0.4081 & 0.5180 & 0.2175 & 0.3610 & 0.2411 & 0.4374 & 0.4297 & 0.5301 & 0.6026 \\
% eng-twi   & 0.7306 & 0.7309 & 0.7468 & 0.3578 & 0.5657 & 0.4553 & 0.6777 & 0.6856 & 0.6966 & 0.7500 \\
% eng-kin   & 0.6455 & 0.6946 & 0.6974 & 0.2399 & 0.4975 & 0.6815 & 0.6189 & 0.7384 & 0.7286 & 0.7722 \\
% eng-amh   & 0.5488 & 0.4474 & 0.5865 & 0.5565 & 0.5931 & 0.6127 & 0.6189 & 0.6387 & 0.6021 & 0.6252 \\
% eng-yor   & 0.4890 & 0.5854 & 0.5945 & 0.1411 & 0.4740 & 0.5399 & 0.5015 & 0.5243 & 0.5441 & 0.6111 \\
% eng-hau   & 0.2448 & 0.3923 & 0.3824 & 0.2114 & 0.3580 & 0.4141 & 0.4049 & 0.4156 & 0.3854 & 0.4452 \\
% \midrule
% Average  & 0.5537 & 0.5512 & 0.6000 & 0.2705 & 0.4877 & 0.4273 & 0.5449 & 0.4972 & 0.5965 & \textbf{0.6565} \\
% \bottomrule
% \end{tabular}
% }
% \caption{Pearson correlation of quality estimation (QE) systems across selected language pairs.}
% \label{tab:qe_pearson}
% \end{table*}

\begin{table*}[htbp]
\centering
\large
\setlength\tabcolsep{4pt}
\resizebox{1.05\textwidth}{!}{%
\begin{tabular}{c|ccccc|cc|cc}
\toprule
\makecell[l]{LP} & \textbf{COMETKIWI} & 
\makecell[c]{\textbf{AfriCOMET} \\ \textbf{v1.1 STL}} & 
\makecell[c]{\textbf{AfriCOMET} \\ \textbf{v1.0 MTL}} & 
\makecell[c]{\textbf{AfriCOMET} \\ \textbf{v1.1 MTL}} & 
\textbf{Metric-X 24} & 
\textbf{Claude-3.7} & 
\makecell[c]{\textbf{Gemini-2.5} \\ \textbf{pro}} & 
\makecell[c]{\textbf{SSA-COMET} \\ \textbf{STL}} & 
\makecell[c]{\textbf{SSA-COMET} \\ \textbf{MTL}} \\
\midrule
\texttt{eng-amh} & 0.556 & 0.593 & 0.613 & 0.619 & 0.639 & 0.587 & 0.593 & 0.596 & 0.625 \\
\texttt{eng-hau} & 0.211 & 0.358 & 0.414 & 0.405 & 0.416 & 0.382 & 0.412 & 0.393 & 0.442 \\
\texttt{eng-kik} & 0.299 & 0.582 & 0.377 & 0.648 & 0.452 & 0.609 & 0.650 & 0.657 & 0.730 \\
\texttt{eng-kin} & 0.240 & 0.497 & 0.681 & 0.619 & 0.738 & 0.694 & 0.714 & 0.735 & 0.788 \\
\texttt{eng-luo} & 0.176 & 0.560 & 0.259 & 0.638 & 0.332 & 0.646 & 0.721 & 0.649 & 0.728 \\
\texttt{eng-twi} & 0.358 & 0.566 & 0.455 & 0.678 & 0.686 & 0.747 & 0.771 & 0.698 & 0.753 \\
\texttt{eng-yor} & 0.141 & 0.474 & 0.540 & 0.501 & 0.524 & 0.595 & 0.607 & 0.547 & 0.617 \\
\texttt{fra-ewe} & 0.218 & 0.361 & 0.241 & 0.437 & 0.430 & 0.518 & 0.524 & 0.533 & 0.608 \\
\texttt{fra-wol} & 0.236 & 0.399 & 0.264 & 0.358 & 0.258 & 0.623 & 0.676 & 0.583 & 0.649 \\
\texttt{por-vmw} & 0.088 & 0.165 & 0.219 & 0.168 & 0.369 & 0.551 & 0.528 & 0.281 & 0.295 \\
\midrule
Average & 0.252 & 0.455 & 0.406 & 0.507 & 0.484 & 0.595 & 0.620 & 0.567 & \textbf{0.623} \\
\bottomrule
\end{tabular}
}
\caption{Pearson correlation of QE metrics across language pairs.}
\label{tab:qe_pearson_3dp}
\end{table*}




==> tables/main_results_QE_Spearman.tex <==
% \begin{table*}[htbp]
% \centering
% \large
% \resizebox{1.05\textwidth}{!}{%
% \begin{tabular}{l|ccc|ccccc|cc}
% \toprule
% \makecell[l]{Language\\Pair}  & \makecell[c]{Gemini-2.0\\flash} & \makecell[c]{GPT-4o\\5shots} & \makecell[c]{Claude-3.7\\5shots} & CometKiwi & AfriCOMETv1.1-QE & AfriCOMETv1.0-MTL & AfriCOMETv1.1-MTL & Metric-X24 & SSA-COMET-QE & SSA-COMET-MTL \\
% \midrule
% eng-kik & 0.6598 & 0.6115 & 0.6773 & 0.3385 & 0.5920 & 0.3849 & 0.6547 & 0.4644 & 0.6912 & \textbf{0.7369} \\
% eng-luo & 0.6434 & 0.6219 & 0.6717 & 0.1841 & 0.5713 & 0.2330 & 0.6437 & 0.3295 & 0.6561 & 0.7319 \\
% fra-wol & 0.7053 & 0.6567 & 0.6874 & 0.3071 & 0.4337 & 0.2724 & 0.4069 & 0.2914 & 0.6336 & 0.6800 \\
% fra-ewe & 0.5913 & 0.4193 & 0.5922 & 0.2447 & 0.3697 & 0.2248 & 0.4827 & 0.4763 & 0.5690 & 0.6274 \\
% eng-twi & 0.6013 & 0.5983 & 0.6396 & 0.3461 & 0.4576 & 0.3141 & 0.5608 & 0.5632 & 0.6079 & 0.6549 \\
% eng-kin & 0.4481 & 0.5047 & 0.5298 & 0.1665 & 0.3973 & 0.4995 & 0.4726 & 0.5917 & 0.5136 & 0.5553 \\
% eng-amh & 0.4912 & 0.3915 & 0.5406 & 0.4943 & 0.5474 & 0.5743 & 0.5685 & 0.6181 & 0.5565 & 0.5905 \\
% eng-yor & 0.3292 & 0.4279 & 0.4924 & 0.0768 & 0.3737 & 0.4334 & 0.4237 & 0.4045 & 0.4473 & 0.5191 \\
% eng-hau & 0.2119 & 0.3299 & 0.3565 & 0.1852 & 0.3505 & 0.4015 & 0.3882 & 0.4361 & 0.3803 & 0.4359 \\
% \midrule
% Average & 0.5202 & 0.5069 & 0.5764 & 0.2604 & 0.4548 & 0.3709 & 0.5113 & 0.4639 & 0.5617 & \textbf{0.6147} \\
% \bottomrule
% \end{tabular}
% }
% \caption{Spearman correlation of quality estimation (QE) systems across selected language pairs.}
% \label{tab:qe_spearman}
% \end{table*}

\begin{table*}[htbp]
\centering
\large
\setlength\tabcolsep{4pt}
\resizebox{1.05\textwidth}{!}{%
\begin{tabular}{c|ccccc|cc|cc}
\toprule
\makecell[l]{LP} & \textbf{COMETKIWI} & 
\makecell[c]{\textbf{AfriCOMET} \\ \textbf{v1.1 STL}} & 
\makecell[c]{\textbf{AfriCOMET} \\ \textbf{v1.0 MTL}} & 
\makecell[c]{\textbf{AfriCOMET} \\ \textbf{v1.1 MTL}} & 
\textbf{Metric-X 24} & 
\textbf{Claude-3.7} & 
\makecell[c]{\textbf{Gemini-2.5} \\ \textbf{pro}} & 
\makecell[c]{\textbf{SSA-COMET} \\ \textbf{STL}} & 
\makecell[c]{\textbf{SSA-COMET} \\ \textbf{MTL}} \\
\midrule
\texttt{eng-amh} & 0.494 & 0.547 & 0.574 & 0.568 & 0.618 & 0.541 & 0.558 & 0.552 & 0.591 \\
\texttt{eng-hau} & 0.185 & 0.350 & 0.401 & 0.388 & 0.436 & 0.357 & 0.401 & 0.390 & 0.428 \\
\texttt{eng-kik} & 0.339 & 0.592 & 0.385 & 0.655 & 0.464 & 0.677 & 0.703 & 0.685 & 0.734 \\
\texttt{eng-kin} & 0.166 & 0.397 & 0.500 & 0.473 & 0.592 & 0.530 & 0.534 & 0.511 & 0.561 \\
\texttt{eng-luo} & 0.184 & 0.571 & 0.233 & 0.644 & 0.329 & 0.672 & 0.757 & 0.653 & 0.728 \\
\texttt{eng-twi} & 0.346 & 0.458 & 0.314 & 0.561 & 0.563 & 0.640 & 0.697 & 0.614 & 0.659 \\
\texttt{eng-yor} & 0.077 & 0.374 & 0.433 & 0.424 & 0.405 & 0.492 & 0.531 & 0.447 & 0.529 \\
\texttt{fra-ewe} & 0.245 & 0.370 & 0.225 & 0.483 & 0.476 & 0.592 & 0.623 & 0.572 & 0.632 \\
\texttt{fra-wol} & 0.307 & 0.434 & 0.272 & 0.407 & 0.291 & 0.687 & 0.743 & 0.638 & 0.689 \\
\texttt{por-vmw} & 0.090 & 0.120 & 0.156 & 0.134 & 0.292 & 0.498 & 0.481 & 0.199 & 0.237 \\
\midrule
Average & 0.243 & 0.421 & 0.349 & 0.474 & 0.447 & 0.569 & 0.603 & 0.526 & 0.579 \\
\bottomrule
\end{tabular}
}
\caption{Spearman correlation of QE metrics across language pairs. All scores rounded to 3 decimal places.}
\label{tab:qe_spearman_3dp}
\end{table*}



==> tables/newdataonlyVsWithWMT_unified.tex <==
\begin{table}[htbp]
\centering
\scriptsize
\setlength\tabcolsep{4pt}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|cc|cc|cc|cc}
\toprule
\multirow{2}{*}{\textbf{LP}} 
& \multicolumn{4}{c|}{\textbf{SSA-COMET-STL}} 
& \multicolumn{4}{c}{\textbf{SSA-COMET-MTL}} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9}
& \multicolumn{2}{c|}{w/o WMT Data} & \multicolumn{2}{c|}{w/ WMT Data}
& \multicolumn{2}{c|}{w/ WMT Data} & \multicolumn{2}{c}{w/ WMT Data} \\
& \textbf{Spear.} & \textbf{Pear.} & \textbf{Spear.} & \textbf{Pear.} 
& \textbf{Spear.} & \textbf{Pear.} & \textbf{Spear.} & \textbf{Pear.} \\
\midrule
eng-amh  & 0.558 & 0.590 & 0.597 & 0.627 & 0.587 & 0.615 & 0.629 & 0.660 \\
eng-hau  & 0.442 & 0.455 & 0.459 & 0.467 & 0.425 & 0.426 & 0.502 & 0.514 \\
eng-kik  & 0.716 & 0.708 & 0.715 & 0.693 & 0.757 & 0.750 & 0.765 & 0.764 \\
eng-kin  & 0.592 & 0.743 & 0.584 & 0.766 & 0.554 & 0.777 & 0.602 & 0.798 \\
eng-luo  & 0.697 & 0.690 & 0.689 & 0.680 & 0.736 & 0.733 & 0.773 & 0.770 \\
eng-twi  & 0.645 & 0.714 & 0.649 & 0.728 & 0.662 & 0.748 & 0.700 & 0.776 \\
eng-yor  & 0.494 & 0.579 & 0.489 & 0.573 & 0.530 & 0.603 & 0.558 & 0.640 \\
fra-ewe  & 0.658 & 0.621 & 0.599 & 0.542 & 0.638 & 0.600 & 0.670 & 0.644 \\
fra-wol  & 0.682 & 0.637 & 0.664 & 0.612 & 0.705 & 0.673 & 0.732 & 0.709 \\
por-vmw  & 0.288 & 0.358 & 0.280 & 0.369 & 0.262 & 0.317 & 0.327 & 0.410 \\
\midrule
\textbf{Average} 
& \textbf{0.577} & \textbf{0.609} & \textbf{0.573} & \textbf{0.606} 
& \textbf{0.586} & \textbf{0.624} & \textbf{0.626} & \textbf{0.668} \\
\bottomrule
\end{tabular}
}
\caption{Spearman and Pearson correlations for SSA-COMET models trained on new data only or with WMT training data.}
\label{tab:ssa-comet-aligned}
\end{table}


==> tables/spearman_main.tex <==
\begin{table*}[!t]
\begin{center}
\centering
% \resizebox{2\columnwidth}{!}{%
\scalebox{0.6}{
\begin{tabular}{l|cc|c|c|c|ccc|c}
\toprule
& \multicolumn{2}{c|}{\textbf{N-gram Matching}} 
& \multicolumn{1}{c|}{\textbf{Embedding-based}} 
& \multicolumn{1}{c|}{\textbf{LLM Prompting}}
& \multicolumn{5}{c}{\textbf{Learned COMET Metrics}} \\
\cmidrule{2-10}
& \multicolumn{1}{c}{\multirow{2}{*}{SacreBLEU}} 
& \multicolumn{1}{c|}{\multirow{2}{*}{chrf++}}
& \multicolumn{1}{c|}{\multirow{2}{*}{BERTScore}}
& \multicolumn{1}{c|}{\multirow{2}{*}{GPT-4}} 
& \textbf{Baseline} 
& \multicolumn{3}{c|}{\textbf{Single Task} (Ours)} 
& \textbf{Multi Task} (Ours) \\
\cmidrule{6-10}
LP & & & & & COMET22 & XLM-R-L & InfoXLM-L & AfroXLM-R-L \ding{72} & AfroXLM-R-L \ding{72} \\
\midrule
ary-fra	&	0.332	&	0.328	&	0.351	&	\textbf{0.620}	&	0.533	&	0.551	&	\textbf{0.565}	&	\textbf{0.567}	&	\textbf{0.609}	\\
eng-arz	&	0.324	&	0.321	&	0.355	&	0.509	&	0.503	&	0.486	&	0.488	&	0.532	&	\textbf{0.600}	\\
eng-fra	&	0.246	&	0.280	&	0.282	&	\textbf{0.536}	&	\textbf{0.489}	&	\textbf{0.510}	&	0.460	&	\textbf{0.495}	&	\textbf{0.526}	\\
eng-hau	&	0.200	&	0.301	&	0.404	&	0.378	&	0.430	&	0.401	&	0.334	&	0.515	&	\textbf{0.620}	\\
eng-ibo	&	0.339	&	0.424	&	0.403	&	0.271	&	0.373	&	0.413	&	0.377	&	\textbf{0.592}	&	\textbf{0.616}	\\
eng-kik	&	0.273	&	\textbf{0.295}	&	0.276	&	0.269	&	0.202	&	0.281	&	0.249	&	\textbf{0.389}	&	\textbf{0.410}	\\
eng-luo	&	0.182	&	0.279	&	\textbf{0.365}	&	0.246	&	0.062	&	0.201	&	0.241	&	\textbf{0.283}	&	\textbf{0.359}	\\
eng-som	&	0.161	&	0.279	&	0.345	&	0.281	&	0.474	&	0.466	&	0.420	&	\textbf{0.554}	&	\textbf{0.546}	\\
eng-swh	&	0.481	&	0.565	&	0.701	&	\textbf{0.774}	&	\textbf{0.738}	&	\textbf{0.739}	&	\textbf{0.719}	&	0.688	&	\textbf{0.733}	\\
eng-twi	&	\textbf{0.204}	&	\textbf{0.178}	&	0.111	&	\textbf{0.132}	&	0.096	&	0.103	&	\textbf{0.112}	&	\textbf{0.157}	&	0.101	\\
eng-xho	&	0.090	&	\textbf{0.161}	&	\textbf{0.168}	&	\textbf{0.143}	&	0.071	&	0.070	&	0.059	&	\textbf{0.191}	&	\textbf{0.146}	\\
eng-yor	&	0.210	&	0.204	&	0.250	&	\textbf{0.446}	&	0.150	&	0.193	&	0.191	&	0.287	&	0.365	\\
eng-yor (it)	&	0.295	&	0.346	&	\textbf{0.421}	&	\textbf{0.447}	&	0.334	&	0.256	&	0.268	&	0.266	&	\textbf{0.418}	\\
eng-yor (movie)	&	0.238	&	0.221	&	0.303	&	\textbf{0.544}	&	0.334	&	0.338	&	0.364	&	0.372	&	0.390	\\
eng-yor (news)	&	0.114	&	0.122	&	0.111	&	\textbf{0.200}	&	\textbf{0.168}	&	\textbf{0.196}	&	\textbf{0.132}	&	\textbf{0.200}	&	\textbf{0.211}	\\
eng-yor (ted)	&	0.027	&	0.002	&	0.091	&	\textbf{0.237}	&	0.123	&	0.177	&	\textbf{0.263}	&	\textbf{0.324}	&	\textbf{0.298}	\\
yor-eng	&	0.308	&	0.408	&	0.446	&	\textbf{0.476}	&	\textbf{0.502}	&	0.460	&	\textbf{0.481}	&	\textbf{0.490}	&	\textbf{0.541}	\\
\midrule
Avg.	&	0.237	&	0.277	&	0.317	&	0.383	&	0.328	&	0.344	&	0.337	&	\textbf{0.406}	&	\textbf{0.441}	\\
\bottomrule
\end{tabular}
}
\end{center}
\caption{Sentence-level Spearman-rank correlation coefficients for MT evaluation models.
%Values with $^*$ indicate a p-value greater than 0.05. 
For each LP, values in~\textbf{bold} represent the highest ranking obtained from the Perm-Input hypothesis test~\citep{deutsch2021statistical}. Comprehensive results of this test are detailed in Table~\ref{tab:spearman_main_rank}. Averaged Spearman-rank correlations across LPs are presented in the last row.}
\label{tab:spearman_main_result}
\vspace{-0.5cm}
\end{table*}
